Effective and secure federated online learning to rank

Online Learning to Rank (OLTR) optimises ranking models using implicit user feedback, such as clicks. Unlike traditional Learning to Rank (LTR) methods that rely on a static set of training data with relevance judgements to learn a ranking model, OLTR methods update the model continually as new data arrives. Thus, it addresses several drawbacks such as the high cost of human annotations, potential misalignment between user preferences and human judgments, and the rapid changes in user query intents. However, OLTR methods typically require the collection of searchable data, user queries, and clicks, which poses privacy concerns for users. Federated Online Learning to Rank (FOLTR) integrates OLTR within a Federated Learning (FL) framework to enhance privacy by not sharing raw data. While promising, FOLTR methods currently lag behind traditional centralised OLTR due to challenges in ranking effectiveness, robustness with respect to data distribution across clients, susceptibility to attacks, and the ability to unlearn client interactions and data. This thesis presents a comprehensive study on Federated Online Learning to Rank, addressing its effectiveness, robustness, security, and unlearning capabilities, thereby expanding the landscape of FOLTR.

==> Chapter3_effective/paper1_foltres_ecir2021/sections/related_works.tex <==
\section{Related Work}

Learning to rank (LTR) consists of the application of supervised machine learning techniques to learn a ranking function from a set of labelled query-document pair examples, represented by features. A key limitation of LTR is the reliance on explicit relevance annotations (labels), which require substantial effort and cost to collect~\cite{DBLP:journals/corr/QinL13,DBLP:journals/jmlr/ChapelleC11}. Editorial labelling also poses ethical issue when needing labels for private data~\cite{wang2016learning}, e.g., emails; in addition user preferences may not agree with that of annotators~\cite{sanderson2010test} and these labels cannot reflect evolving user preferences and search intents~\cite{lefortier2014online}.

The use of implicit feedback in the form of, e.g., clicks has been suggested as a way to go beyond the above limitations~\cite{joachims2002optimizing}; this is the type of signal that the methods studied in this paper consider. 
This setting however presents a number of challenges: clicks are affected by a number of biases and noise, e.g., position bias and noisy clicks~\cite{guan2007eye,joachims2017unbiased,pan2007google}. Approaches that exploit click feedback can be divided into counterfactual learning to rank (CLTR)~\cite{joachims2017unbiased} and online learning to rank (OLTR) \cite{yue2009interactively}. CLTR relies on historical click through logs, treated as pure binary relevance labels, and commonly inverse propensity scoring (IPS) is used to re-weight clicks to minimise the impact of biases. Rankers are then trained in an offline manner and deployed online after training. 
OLTR instead, interactively updates rankers after each user interaction, in an online manner, and rankers explicitly manipulate SERPs to guide the learning process. This is the setup we consider in this paper, where rankers are iteratively updated in an online fashion following user interactions. A key aspect of OLTR is that the online interventions performed by rankers to guide the learning process carry the risk of displaying non optimal SERPs directly to the user, thus hurting user experience. It is important then for OLTR to rapidly learn a high quality ranker so as to not displaying low quality SERPs to a large number of users.

Little attention has been put on the fact that OLTR requires the search engine to monitor and collect user behaviour, thus not being appropriate when users want to preserve their privacy. In fact, current OLTR methods consider a central server that produces SERPs, collects queries and implicit user feedback, and updates a central ranker. An exception is the work of Kharitonov~\cite{kharitonov2019federated}, considered in this paper, that instead exploits federate learning to de-centralise the collection of user data and computation of gradient updates to the ranker; a central server is still required, but this only observes the federated gradient updates, which are then applied to the central ranker which is then distributed to the clients at each update iteration (more details in Section~\ref{sec:method}). Federated (machine) learning was recently introduced by Konecny et al.~\cite{DBLP:journals/corr/KonecnyMRR16,DBLP:journals/corr/KonecnyMYRSB16}; in this framework models are learnt based on datasets distributed across different locations (clients) without the need to share the actual data, and with mechanisms to guarantee data leakage~\cite{yang2019federated}. 
Privacy preservation is a topic of growing interest in information retrieval, with related workshops and tutorials being held in relevant venues~\cite{yang2016privacy,yang2017differential}, but its main focus so far has been on query log anonymisation and privacy-preservation when sharing logs~\cite{cooper2008survey,korolova2009releasing,zhang2016anonymizing}, rather than on integrating privacy preservation mechanisms within the ranking algorithms, as the work of Kharitonov instead does~\cite{kharitonov2019federated}.

==> Chapter3_effective/paper2_fpdgd_ictir2021/sections/related_works.tex <==
\label{sec:relatect works} 
\section{Related works}

\subsubsection*{\textbf{OLTR}} 
Online Learning to Rank (OLTR) differs from traditional Learning to Rank (LTR) methods in that it makes use of user online feedback (such as clicks) as the optimization goal in order to tackle some data-annotation drawbacks of LTR. In fact, LTR relies on explicit relevance annotations (labels), which often imply high annotation costs. In addition, editorial annotation may be of ethical concern when private data, such as emails, need to be labelled~\cite{wang2016learning}. Furthermore, user preferences may not agree with that of annotators~\cite{sanderson2010test}, users' search intents may change from time to time~\cite{lefortier2014online,zhuang2021how}, and explicit relevance labels may not account for these aspects.

The Dueling Bandit Gradient Descent (DBGD) uses online evaluation to unbiasedly compare two or more rankers given a user interaction~\cite{yue2009interactively}. Subsequent work developed more reliable or more efficient online evaluation methods, including Probabilistic Interleaving (PIGD)~\cite{hofmann2011probabilistic}, and its extension, the Probabilistic Multileaving (PMGD)~\cite{oosterhuis2016probabilistic}, which compares multiple rankers at each interaction, resulting in the best DBGD-based algorithm. However, this method suffers from a high computational cost because it requires sampling ranking assignments to infer outcomes~\cite{zhuang2020counterfactual}. Further variations that reuse historical interaction data to accelerate the learning in DBDG have also been investigated~\cite{hofmann2013reusing}.

The Pairwise Differentiable Gradient Descent method (PDGD)~\cite{Oosterhuis2018Unbiased} constructs a pairwise gradient to update the ranking model according to the click feedback. Compared to previous OLTR methods, PDGD has showcased faster learning (higher online nDCG) and convergence to higher effectiveness (higher offline nDCG). Unlike other methods, PDGD can be applied to any differentiable ranking model and it is an unbiased method. Oosterhuis and de Rijke trained a linear and a neural ranker and both showed effective results~\cite{Oosterhuis2018Unbiased}. PDGD is the current state-of-the-art OLTR method.

\subsubsection*{\textbf{Federated learning with privacy protection}} 
\emph{Federated Learning}~\cite{mcmahan2017communication} considers a  machine learning setting where several data owners (clients) collaboratively train a model without sharing the data. To this aim, a coordinator (central server) is required and each participating client sends what is essential for the training (for example, the local gradient) to the central server. The Federated Averaging (FedAvg) algorithm~\cite{mcmahan2017communication} relies on local stochastic gradient descent (SGD), which is computed by each client, while the centralised server performs the global model update by weighted averaging the client's updates.

Differential privacy~\cite{dwork2006calibrating,dwork2014algorithmic} is a method often used to ensure user privacy preservation in federated learning (the alternative is the encryption of the messages). We shall review the notion of  $\epsilon$-differential privacy in Section~\ref{dp}. Abadi et al.~\cite{abadi2016deep} have developed the algorithmic techniques for combining SGD-based deep learning methods with differential privacy. Differential privacy has also been added to FedAvg algorithm to provide user-level differential privacy guarantees for language models~\cite{mcmahan2018learning}, as for these models it has been shown that the gradients or shared model's weights can reveal sensitive information regarding the clients' data~\cite{fredrikson2015model, shokri2017membership, geiping2020inverting}. 

\subsubsection*{\textbf{Federated OLTR}} 
OLTR has been primarily investigated in a centralised paradigm, where a central server holds the data to be searched and collects the users' search interactions (e.g., queries, clicks). The training of the ranker is also conducted by the server. This centralised paradigm is not suited to a privacy-preserving situation where each client does not want to share the data on which it wants to search, along with queries and other search interactions.

Recently, the Federated OLTR with Evolutionary Strategies method (FOLtR-ES)~\cite{kharitonov2019federated} has been proposed to address the above privacy-preserving issues. FOLtR-ES extends the OLTR optimization scenario to the Federated SGD~\cite{mcmahan2017communication} and uses Evolution Strategies as the optimization method~\cite{salimans2017evolution}. To defend the gradient updates from a malicious attacker, FOLtR-ES also includes a privatization procedure, which leverages the theory of $\epsilon$-local differential privacy~\cite{dwork2014algorithmic}. FOLtR-ES is shown to perform well on small-scale datasets (MQ2007) for the MaxRR metric, although performance degrades when privacy preservation is required~\cite{kharitonov2019federated}. However, the effectiveness of FOLtR-ES is not consistent across other, larger-scale datasets nor when typical OLTR metrics are considered (nDCG)~\cite{wang2021federated}. 


==> Chapter4_paper2_noniid_sigir2022/sections/experimental_setup.tex <==
\section{Preliminaries: Common experiment settings}
\label{experiment}
Next, we describe the settings that are in common among the experiments we execute to understand the impact of different types of non-IID data and to posit what problems future research in the emerging area of FOLTR should tackle. For most experiments, with respect to the use standard learning to rank datasets (except in one occasion), the simulation of user interactions with SERPs, and the measurement of both online and offline performance, we rely on the typical evaluation setup used in OLTR~\cite{hofmann2013fast, oosterhuis2016probabilistic, oosterhuis2018differentiable} with the adaptations made by \citet{wang2021effective} for the federated setting.

%Same as~\cite{wang2021effective}, we rely on the typical evaluation setup used by previous OLTR research~\cite{hofmann2013fast, oosterhuis2016probabilistic, oosterhuis2018differentiable} to empirically investigate the impact of non-IID data to the FPDGD approach, and how it compares to the IID settings. This consists of use standard learning to rank datasets, simulate user interactions with SERPs, i.e. simulate clicks, and measure both online and offline performance.


\textbf{Datasets.}
For most experiments we consider three publicly available LTR datasets: MSLR-WEB10k~\cite{qin2013introducing} (10,000 queries), Yahoo~\cite{chapelle2011yahoo} (29,900 queries) and Istella-S~\cite{lucchese2016post} (33,018 queries). Each dataset consists of a set of queries and the corresponding preselected document set: every query-document pair is represented by a feature vector and the annotated relevance label. These three commercial datasets are all annotated for relevance on a five-grade-scale: from \emph{not relevant} (0) to \emph{perfectly relevant} (4).
%While other, larger datasets for learning to rank are currently available, our choice considered the trade-off between representativeness and the high computational costs associated with experimenting with the federated OLTR methods on larger datasets.

%The three LTR datasets we consider are all provided by commercial search engines. The MSLR-WEB10k, constructed from a retired labelling set of the Microsoft web search engine, contains 10,000 queries (divided into 5 folds), and on average each query is associated with 125 documents. The Yahoo dataset is sampled from a query log of the Yahoo! search engine. It contains approximately 29,900 queries and each query-document pair is represented by 700 features. Lastly, the Istella-S dataset is the largest dataset we consider, with 33,018 queries, 220 features, and an average of 103 documents per query. These three commercial datasets are all annotated for relevance on a five-grade-scale: from \emph{not relevant} (0) to \emph{perfectly relevant} (4).

From the above datasets, we synthetically construct non-IID partitions of the datasets according to specific criteria (depending on the non-IID data types described afterwards). This synthetic process of construction was required because: (1) no currently available LTR dataset clearly exhibits non-IID characteristic, (2) synthetic strategies allow to easily quantify and control the amount of imbalance across the local data in each client, (3) prior knowledge derived from prior work on centralised training (i.e. non-federated) can be leveraged as reference or baselines.

%We choose to synthetise the distributed non-IID datasets for our experiments by partitioning the aforementioned datasets from commercial search engines into multiple subsets. The reasons for using synthetic datasets instead of real-world non-IID datasets are as follows. First of all, there is lack of real-world non-IID datasets for OLTR tasks. Second, synthetic strategies can easily quantify and control the imbalance degree of the local data comparing to real-world datasets. Third, it is more flexible to develop synthetic strategies on existing widely used public datasets. For example, different numbers of clients can be set to simulate different scenarios. However, in real-world non-IID dataset, the number of clients tends to be fixed thus limit the experimentation. Lastly, for widely-used IID datasets, more prior knowledge from centralised training can be leveraged as reference or baselines.

\textbf{User simulations.}
%It is common practice in OLTR to use LTR datasets and simulate user interactions as no public dataset with LTR features and clicks is available. 
%Following previous work in OLTR~\cite{hofmann2013fast, oosterhuis2016probabilistic, Oosterhuis2018Unbiased}, we simulate users and their reaction with the search results using labeled offline learning to rank datasets. 
Both querying and clicking behaviours were simulated. 

For the querying behaviour, for each client participating in the federated OLTR, we sample $B$ queries randomly, in line with previous work on FOLTR~\cite{kharitonov2019federated, wang2021effective}. For each query, we use the local ranking model (i.e. that held by the client) to rank documents; we limit SERP to 10 documents. 

For the click behaviour, we rely on the \emph{Simplified Dynamic Bayesian Network} (SDBN) click mode~\cite{chapelle2009dynamic}. Under SDBN, users are assumed to examine a SERP from top to bottom. Each document is inspected and clicked with click probability $P(click = 1 | R)$, conditioned on the relevance label $R = rel(d)$. After a click occurs, the user stops scanning with stopping probability $P(stop = 1 | R)$, or continues otherwise. It is common practice in OLTR to consider three instantiations of the SDBN: a \textit{perfect} user with very reliable feedback, a \textit{navigational} user searching for reasonably relevant documents, and an \textit{informational} user with the noisiest click feedback among the three instantiations. The values used for $P(click = 1 | R)$ and $P(stop = 1 | R)$ for SDBN in all considered datasets are reported in Table~\ref{tbl:sdbn}. In the study of click preference skewness (Section~\ref{noniid:cps}), we also adopt the \emph{Position-Based Model} (PBM)~\cite{craswell2008experimental}, which considers the probability that the user examines a document is highly relevant to the rank or position of the document on a SERP (search engine result page). The probability of examining typically decreases with the rank and the degree of decreasing is parameterized by $\eta$. The larger value of $\eta$ represents higher decreasing degree, which brings about higher position bias.

%\textbf{non-IID data generation.}

%\textbf{IID baselines.}


\textbf{Ranking models.} 
We choose both a linear and neural model as the ranking models when training with FPDGD. For the linear ranking model, we set the learning rate $\eta = 0.1$ and zeor initialization was used. Same as the original paper of PDGD~\cite{oosterhuis2018differentiable}, the neural ranker is optimized by a single hidden-layer neural network with 64 hidden nodes and sigmoid activation functions with \emph{Xavier} initialization~\cite{glorot2010understanding}. We set the learning rate $\eta = 0.1$ for the neural ranker as well.


\textbf{Federated setup.}
We simulate the federated OLTR scenario as follows. Each client holds a copy of the current ranker. For each client, we consider $|B|$ user queries along with the respective interactions, during which the local ranker is optimised using the simulated user clicks. After $|B|$ interactions have occurred, the client sends the local message (gradient update) to the central server. The central server optimises the global ranker by aggregating the local messages and sends the newly-updated ranker back to each client. %In our experiments, we set the number of clients participating in the federated process to 10 and each client conducts 4 queries ($n\_clients = 10, B = 4$).

In our experiments on all datasets, unless otherwise specified, we simulate $ |C| $ clients with each client performing $|B| \in \{2 ,5, 10\}$ interactions (queries) locally to contribute to each global model update. We restrict the global communication times $T = 10,000$.


\textbf{Evaluation measures.} We rely on previous evaluation practices in OLTR and FOLTR~\cite{oosterhuis2018differentiable,wang2021federated,wang2021effective}. To measure offline performance, we average nDCG@10 of the global ranker over the queries in the held-out test set. We record this performance value after each update of the global ranker and the final performance is also recorded. To measure online performance, we compute the cumulative discounted nDCG@10 (with $\gamma = 0.9995$) for the rankings displayed during the training phase~\cite{hofmann2013fast}. 
%To evaluate FOLTR methods we rely on the evaluation practice from previous OLTR work, which consists of measuring the rankers' offline and online performance.

%As FOLTR update the global ranker based on clients' online feedback, we divide our evaluation into two parts: offline evaluation and online evaluation.

%To measure offline performance, we average nDCG@10 of the global ranker over the queries in the held-out test set. We record this performance value after each update of the global ranker and the final performance is also recorded. %We consider $k = 10$ as the number of documents in a ranked list for a query. 

%The NDCG@k score is calculated based on formula below:
%\begin{equation}
%NDCG@k = \sum_{i = 1}^{k}\frac{2^{rel(r[i])} - 1}{log_2(i + 1)} iDCG^{-1}
%\end{equation}
%This metric calculates the Discounted Cumulative Gain (DCG) using the relevance labels $rel(r[i])$ for each document in the top $k$ ranking list. For a fair comparison between different queries, the DCG score is normalized by the ideal DCG (iDCG), that is the potentially maximal DCG for one query. 
%
%To measure online performance, we compute the cumulative discounted nDCG@10 (with $\gamma = 0.9995$) for the rankings displayed during the training phase~\cite{hofmann2013fast}. 
%%For $t$-th query in a sequence of $T$ queries, with $R^t$ representing the ranking list displayed to the user, online performance is computed as:
%%\begin{equation}
%%	\label{eq:onlinemetric}
%%	Online\_Performance = \sum_{t = 1}^{T}nDCG(R^t)\cdot\gamma^{t-1} \text{.}
%%\end{equation}
%%This measure indicates the quality of the user experience during training; the discount factor $\gamma$ puts more importance to the interactions in the early phases of training. Following previous work~\cite{oosterhuis2018differentiable}, we set $\gamma = 0.9995$.
%
%%All evaluation results are averaged over all dataset training folds and statistical significant differences between system pairs are evaluated using two-tailed Student's t-test with Bonferroni correction.

\textbf{Runs repetition and statistical analysis.}
All experiments are repeated 5 times with different random seeds. Results are averaged and a paired, two-tailed Student's t-test is used for significance test.


==> Chapter4_paper2_noniid_sigir2022/sections/method.tex <==
\section{Methods for Dealing with Non-IID data}

%Many works have shown that non-iid data, especially label distribution skew, can cause severe learning divergence to both linear models and neural networks in (horizontal) FL~\cite{}. Current approaches to addressing Non-IID problems in horizontal FL can be classified into three categories: the data based approach, algorithm based approach, and system based approach~\cite{zhu2021federated}.
%
%Intuitively speaking, in the setting of Non-IID, a client trains the local model without sharing information between clients, which may lead to the local model generalizing poorly on the unseen data.
%
%%COPY
%In data based approaches, data sharing and augmentation are two main solutions with state-of-the -art performance.
%
%Existing works: data-sharing, model traveling
%
%For example, some existing works~\cite{zhao2018federated, jeong2018communication} proposes heuristic-based approaches by sharing local device data or create some server-side proxy data.
%
%In another way, ``training a customized model can turn the non-iid problem from a bug to a feature, almost literally - since each client has its own model, the client's identity effectively parameterizes the model, rendering some pathological but degenerate non-iid distributions trivial.''~\cite{kairouz2019advances} However, training single global model for each client can potentially bring the problem of overfitting.
%
%Wang et al.~\cite{wang2019federated} propose the framework using local fine tuning. It begins with the federated training of a single model, and then deploys the model to all clients, where it is personalized by additional training on the local dataset before inference.
%
%
%\subsection{subsection}


%Existing methods. (Findings till now)

%FedProx: effective for document label distribution skew (type 1) but the hyperparameter $\mu$ needs to be carefully tuned for each click model. FedProx has no significant improvement on document preferences skew (type 2). 
%probably because of the limitation of the dataset (because no relevance between the intent for each query). - FedProx limits the weight space by adding the regularization item. However, if no correlation between the intent of queries from one single client, the weight space are chaotic. 

%FedPer: can only be used for neural ranker. The effectiveness ...

\begin{algorithm}[t]
	\caption{PDGD on FedProx~\cite{li2020federated}. \\
		-  set of clients participating training: $C$, each client is indexed by $c$; \\
		-  number of local interactions for client $c$: $n_c$ ($\sum_{c=1}^{|C|}n_c=n$) \\
		-  local interaction set: $B$, model weights: $\theta$.}
	\label{alg:fedprox}
	\begin{algorithmic}
		\SUB{Server executes:}
		\STATE initialize $\theta_0$; scoring function: $f$; learning rate: $\eta$
		\FOR{each round $t = 1, 2, \dots$}
		\FOR{each client $c \in C$ \textbf{in parallel}}
		\STATE $\theta_{t+1}^c, n_c \leftarrow \text{ClientUpdate}(c, \theta_t)$
		\ENDFOR
		\STATE $\theta_{t+1} \leftarrow \sum_{c=1}^{|C|} \frac{n_c}{n} \theta_{t+1}^c$
		\ENDFOR
		\STATE
		
		\SUB{ClientUpdate($c, \theta_{t}$):}\ \ \ // \emph{Run on client $c$}
		\FOR{each local update $i$ from $1$ to $B$}
		\STATE $f_{\theta_{t}}^c \leftarrow f_{\theta_{t}}^* + \frac{\mu}{2}\|\theta - \theta_{t}\|^2$    \hfill \textit{\small //$f_{\theta_{t}}^*$: scoring function from PDGD}
		\STATE $\theta_{t+1}^c \leftarrow \theta_{t} + \eta\nabla f_{\theta_{t}}^c$
		\ENDFOR
		\STATE return ($\theta_{t+1}^c, n_c$) to server
	\end{algorithmic}	
\end{algorithm}	


\begin{figure*}[t]
	\centering
	\subfigure[\textbf{MSLR-WEB10k (linear ranker)}] {\label{fig:mslr-linear-datashare} \includegraphics[width=17cm]{images/MSLR10K_FPDGD_clients5_batch5_updates10000_non_iid_label_dist_skew1_CCM_linear_data_sharing_10percent.png}} 
	\subfigure[\textbf{MSLR-WEB10k (neural ranker)}] {\label{fig:mslr-neural-datashare} \includegraphics[width=17cm]{images/MSLR10K_FPDGD_clients5_batch5_updates10000_non_iid_label_dist_skew1_CCM_neural64_data_sharing_10percent.png}} 
	\vspace{-12pt}
	\caption{Offline performance (nDCG@10) in MSLR-10k datasets for data-sharing, under three instantiations of SDBN click model with local updates setting $B = 5$; results averaged across all dataset splits and experimental runs.
		\label{fig:datashare}}
\end{figure*}


\begin{figure*}[t]
	\centering
	\subfigure[\textbf{MSLR-WEB10k (linear ranker)}] {\label{fig:mslr-linear-fedprox} \includegraphics[width=17cm]{images/MSLR10K_FPDGD_clients5_batch5_updates10000_iid_label_dist_skew_CCM_linear_fedprox.png}} 
	\subfigure[\textbf{intent-change (linear ranker)}] {\label{fig:intent-linear-fedprox} \includegraphics[width=17cm]{images/intent-change_FPDGD_clients4_batch5_updates10000_non_iid_intent_change_CCM_linear_fedprox.png}} 
	\subfigure[\textbf{intent-change (neural ranker)}] {\label{fig:intent-neural-fedprox} \includegraphics[width=17cm]{images/intent-change_FPDGD_clients4_batch5_updates10000_non_iid_intent_change_CCM_neural16_fedprox.png}} 
	\vspace{-12pt}
	\caption{Offline performance (nDCG@10) in MSLR-10k and intent-change datasets for FedProx, under three instantiations of SDBN click model with local updates setting $B = 5$; results averaged across all dataset splits and experimental runs.
	\label{fig:fedprox}}
\end{figure*}


\begin{figure*}[t]
	\centering
	\subfigure[\textbf{MSLR-WEB10k (neural ranker)}] {\label{fig:mslr-neural-fedper} \includegraphics[width=17cm]{images/MSLR10K_FPDGD_clients5_batch5_updates10000_non_iid_label_dist_skew_CCM_neural64_personal.png}} 
	\subfigure[\textbf{intent-change (neural ranker)}] {\label{fig:intent-neural-fedper} \includegraphics[width=17cm]{images/intent-change_FPDGD_clients4_batch5_updates10000_non_iid_intent_change_CCM_neural16_personal.png}} 
	\vspace{-12pt}
	\caption{Offline performance (nDCG@10) in MSLR-10k and intent-change datasets for FedPer, under three instantiations of SDBN click model with local updates setting $B = 5$; results averaged across all dataset splits and experimental runs.
		\label{fig:fedper}}
\end{figure*}


As shown in the last section, the FedAvg algorithm itself can not handle the performance decrease caused by some of the non-IID situations. In this section, we analyse the effectiveness of two state-of-the-art, non-IID targeted FL algorithms (FedProx~\cite{li2020federated} and FedPer~\cite{arivazhagan2019federated}) on FOLTR by directly implementing them to the aforementioned two non-IID types which are shown significant degrading in performance: (1) the document label distribution skewness (type 1), and (2) the document preferences skewness (type 2).

Data-sharing strategy is first proposed by Zhao et al~\cite{zhao2018federated}. According to Zhao et al, the performance reduction is attributed by the weight divergence under different training processes from non-IID data, which is further affected by the divergence between local data distribution and the population distribution. To improve FedAvg with non-IID, a straightforward idea is to slightly reduce the divergence that causes the global model upderperformed. In their strategy, a globally shared dataset $G$ with a population distribution is centralised on the server and a warm-up global model is trained from $G$. Then a random $\alpha$ proportion of $G$ is sent to all connected clients so that the local model is updated by both local training data and the shared data from $G$. Lastly, the server aggregates the local models from the clients and updates the global model with FedAvg. Previous experimental results show that data sharing method can significantly enhance the global model performance on non-IID data. However, the shortcomings are also very obvious. It is very hard to collect uniformly distributed global dataset in the real-world scenario because either the global server need some prior knowledge about the local data distribution or each client needs to share parts of the local data, which violates the privacy requirement of federated learning.

FedProx~\cite{li2020federated} improves the local objective of FedAvg. Specifically, it introduces an additional $L_2$ regularization term in the local objective function to limit the distance between the local model and the global model. In addition, a hyper-parameter $\mu$ is introduced to control the weight of $L_2$ regularization. Our implementation for FedProx on PDGD is shown on Algorithm~\ref{alg:fedprox}. The idea of FedProx is straightforward and only augments little computation overhead. However, main drawback is that the hyper-parameter $\mu$ needs to be carefully tuned to achieve decent results for different tasks. Generally speaking, a large $\mu$ may slow the convergence by forcing the updates to get close to the initial point while a small $\mu$ may not make any difference.

FedPer~\cite{arivazhagan2019federated} aims to solving the statistical heterogeneity (also known as non-IID) in federated learning of deep neural networks by separating them into base layers and personalisation layers. The base layers are trained in a collaborative manner through FedAvg where all clients share the same base layers. Instead, the personalisation layer parts are trained locally from clients' local data with stochastic gradient descent (SGD). This procedure works as follows: after initialisation, each client merges and updates its base and personalised layers locally using a SGD style algorithm. And each client only sends its base layers to the global server. The server updates the globally-shared base layers using FedAvg and sends back again the updated ones to each client. Intuitively, the base layers are updated globally to learn high-level common representations while the distinct personalisation layers never leave the local devices and captures the personalisation aspects of clients. Except for the training and keeping locally of the personalisation layers, FedPer is quite similar as the FedAvg algorithm. Moreover, comparing to FedAvg, FedPer reduces the communication costs as only part of the whole model needs to be transferred and has shown enhancement on learning performance under highly skewed non-IID data for personalisation tasks.

Figure~\ref{fig:datashare} demonstrates the results for data-sharing strategy on MSLR-10k dataset (under label distribution skewness with $\#R = 1$). We randomly select 10\% of the entire dataset as the globally shared data and simulate 5 clients with 5 local updating times before each global updating. It is clearly shown that, with 10\% data-sharing, the global performance can be significantly enhanced for both linear and neural ranker.

Our experimental results on FedProx and FedPer are shown in Figure~\ref{fig:fedprox} and Figure~\ref{fig:fedper} separately. The implementation is conducted on MSLR-10k (under label distribution skewness with $\#R = 1$) and intent-change (under document preferences skewness) datasets. The number of involved clients is set to 5 for MSLR-10k and 4 for intent-change, with both having 5 local updating times before each global updating. For FedProx under different hyper parameter, it is clearly shown that neither of $\mu$ from candidate set $\{0.001, 0.01, 0.1, 1, 10\}$ has higher performance than the original non-IID setting for both linear and neural ranker. Similar results are also concluded from FedPer experiments: there is no significant gain in performance under the neural ranker.

==> Chapter4_paper2_noniid_sigir2022/sections/related_works.tex <==
\section{Related Work}

\subsection{Federated Learning with non-IID data}
Zhu et al. have compiled a comprehensive survey on the impact of non-IID data on federated learning ~\cite{zhu2021federated}, also reviewing the current research on handling these challenges.  
Early work from Zhao et al.~\cite{zhao2018federated} shows a deterioration of the accuracy of federated learning if non-IID or heterogeneous data is present; they also provide a solution to this problem by creating a small subset of globally shared data between all clients (local devices).
Li et al.~\cite{li2020convergence} analyse the convergence of the federated learning algorithm \verb|FedAvg|~\cite{mcmahan2017communication} (which is a component of the FOLTR method we rely upon for investigation~\cite{wang2021effective}) on non-IID data and empirically show that data heterogeneity slows down the convergence. This raised attention to the presence of non-IID data in federated learning. 

Generally speaking, existing approaches for handling non-IID issues in federated learning can be classified into three categories: data-based approaches, algorithm-based approaches, and system-based approaches~\cite{zhu2021federated}.
Data sharing~\cite{zhao2018federated} and data augmentation~\cite{duan2019astraea} are two kinds of typical data-based approaches. While they achieve state-of-the-art performance, they fundamentally conflict with the objective of federated learning: that of not sharing data across clients. This is because, for example, methods such as data sharing require a subset of private data to be shared across all clients. While proposals have been made to use synthetic, rather than real, data for the data sharing mechanism~\cite{wang2021non} it is unclear (1) what the effectiveness loss of the sharing of synthetic data in place of real data is, and (2) whether the sharing of synthetic data could still jeopardise privacy as this synthetic data is typically generated from real data, and thus analysis of the synthetic data may reveal key aspects of and information contained in the real data.
Algorithm-based approaches mainly focus on personalisation methods like local fine-tuning of a neural model~\cite{wang2019federated} and Personalized FedAvg (Per-FedAvg)~\cite{fallah2020personalized} -- which are both limited mainly to neural models -- or the casting of the federated learning process into a multi-task learning problem~\cite{smith2017federated}.
System based approaches adopt clustering~\cite{sattler2020clustered} and tree-based structure~\cite{ghosh2020efficient} to deal with non-IID data.
Limitations exist among all proposed approaches, and this is still a much unexplored line of research.


%COPY
%Federated Learning has recently drawn attention from the LTR community due to growing body of research addressing privacy preservation. Kharitonov~\cite{kharitonov2019federated} studies the federated online LTR and proposed \verb|FOLtR|. Hartmann et al.~\cite{hartmann2019federated} uses FL to solve the URL suggestion task for web browsing experience. Anelli et al.~\cite{anelli2021federank} propose \verb|FedeRank|, which is a FL version of matrix factorization. 

\subsection{Federated Learning in IR}
We provide an overview of the use of federated learning in OLTR in section 3. That section also introduces the FOLTR method used in the empirical experimentation in this paper: the Federated Pairwise Differentiable Gradient Descent (FPDGD) method~\cite{wang2021effective}, which is the current state-of-the-art in FOLTR.

Aside from its usage in OLTR,  recent works have applied federated learning in other IR contexts. Zong et al.~\cite{zong2021fedcmr} provide a solution for cross-modal retrieval in a distributed data storage scenario, which uses federated learning to reduce the potential privacy risks and the high maintenance costs encountered when dealing with a large amount of training data. Wang et al.~\cite{wang2021efficient} study learning to rank (but not OLTR) in a cross-silo federated learning setting; this work is aimed at helping companies that have access to limited labelled data to collaboratively build a document retrieval system efficiently.
Hartmann et al.~\cite{hartmann2019federated} use federated learning to improve the ranking of suggestions
in the Firefox URL bar, so that the training of the ranker on user interactions is performed in a privacy-preserving way; they show that this federated approach improves on the suggestions produced by the previously employed heuristics in Firefox.
Yang et al. ~\cite{yang2018applied} describe the use of federated learning for search query suggestions in the Google Virtual Keyboard (GBoard) product. Here, a baseline model identifies relevant query suggestions given a user query; candidate suggestions are then filtered using a triggering model learnt using federated learning. 
Closest to FOLTR is the work of Li et al.~\cite{li2021federated}, who devise an offline federated learning method for counterfactual learning to rank from historic click logs. %\todo{In general, they propose the FedIPS algorithm, which learns from user interactions on-device with the help of federated learning and uses Inverse Propensity Score (IPS)-weighted Stochastic Gradient Descent (SGD) to compensate the position bias of user interactions for the local updates.}
%\verb|FedIPS|

Aside from the previous examples, federated learning has also seen adoption in the area of personalised search~\cite{ghorab2013personalised}, which aims to return search results that cater to the specific user's interests. While feature-based~\cite{carman2010towards, bennett2012modeling, harvey2013building} and deep learning-based~\cite{song2014adapting, ge2018personalizing, yao2020rlper} methods are widely used in this area, user data privacy has been often overlooked -- this is particularly the case when considering the user's query logs which are collected by the central server to create the personalised ranker. To tackle this issue, Yao et al.~\cite{yao2021fedps} recently proposed a privacy protection enhanced personalised search framework which adapts federated learning to the state-of-the-art personalised search model. While not directly related to the OLTR context we consider here, these related lines of research could benefit from the investigations and considerations reported in this paper, as the problem of non-IID data in these previous contexts has also been ignored.

==> Chapter4_paper2_noniid_sigir2022/sections/results.tex <==
\section{Results Analysis}


Results I want to show:

1. performance gap between non-iid and iid for both online and offline metric in different non-iid settings.

2. hyper-parameters analysis in the non-iid settings. for example, existing works show bigger performance gap when the number of epochs for local updates is large. (from the survey~\cite{zhu2021federated})

==> Chapter5_paper3_poisoning_ictir2023/sections/related-works.tex <==
\section{Related Work}

%\subsection{Online Learning to Rank}
%Online Learning to Rank (OLTR) differs from traditional Learning to Rank (LTR) methods in that it makes use of user online feedback (such as clicks) as the optimization goal in order to tackle some data-annotation drawbacks of LTR. In fact, LTR relies on explicit relevance annotations (labels), which often imply high annotation costs. In addition, editorial annotation may be of ethical concern when private data, such as emails, need to be labelled~\cite{wang2016learning}. Furthermore, user preferences may not agree with that of annotators~\cite{sanderson2010test}, users' search intents may change from time to time~\cite{lefortier2014online,zhuang2021how}, and explicit relevance labels may not account for these aspects.
%
%%The use of implicit feedback in OLTR, however, is often challenging. For example, clicks are affected by noise and a number of biases such as position bias and selection bias~\cite{guan2007tracking, joachims2017unbiased, pan2007google}. 
%
%The Dueling Bandit Gradient Descent (DBGD) uses online evaluation to unbiasedly compare two or more rankers given a user interaction~\cite{yue2009interactively}. Subsequent work developed more reliable or more efficient online evaluation methods, including Probabilistic Interleaving (PIGD)~\cite{hofmann2011probabilistic}, and its extension, the Probabilistic Multileaving (PMGD)~\cite{oosterhuis2016probabilistic}, which compares multiple rankers at each interaction, resulting in the best DBGD-based algorithm. However, this method suffers from a high computational cost because it requires sampling ranking assignments to infer outcomes~\cite{zhuang2020counterfactual}. Further variations that reuse historical interaction data to accelerate the learning in DBDG have also been investigated~\cite{hofmann2013reusing}.
%
%The Pairwise Differentiable Gradient Descent method (PDGD)~\cite{oosterhuis2018differentiable} constructs a pairwise gradient to update the ranking model according to the click feedback. Compared to previous OLTR methods, PDGD has showcased faster learning (higher online performance) and convergence to higher effectiveness (higher offline performance). Unlike other methods, PDGD can be applied to any differentiable ranking model and it is an unbiased method. Oosterhuis and de Rijke trained a linear and a neural ranker and both showed effective results~\cite{oosterhuis2018differentiable}. PDGD is the current state-of-the-art OLTR method.

\subsection{Federated Online Learning to Rank}

Unlike traditional Learning to Rank (LTR), Online Learning to Rank (OLTR) optimizes rankers through implicit user feedback (e.g., clicks) to directly influence search engine result pages in real-time production. The earliest method, Dueling Bandit Gradient Descent (DBGD)~\cite{yue2009interactively}, uniformly samples variations of the ranking model and updates the ranker based on online interleaving evaluation. To mitigate the high variance and regret inherent in DBGD, subsequent methods have improved it through techniques like multiple interleaving~\cite{schuth2016multileave, oosterhuis2017balancing}, projected gradient~\cite{wang2019variance}, and counterfactual evaluation~\cite{zhuang2020counterfactual}. In contrast to DBGD-based approaches, Pairwise Differentiable Gradient Descent (PDGD)~\cite{oosterhuis2018differentiable} utilizes a Plackett-Luce model to sample the ranking list and estimates gradients from inferred pairwise preferences. This method has been found to exhibit greater resilience to noise and higher effectiveness in optimizing neural models.

OLTR methods have been thoroughly investigated in a centralized setting, where a central server possesses the data to be searched and gathers users' search interactions, such as queries and clicks. The training of the ranker also takes place on this server. However, this centralized paradigm is not well-suited for privacy-preserving requirement where each client may not wish to, or cannot, share the searchable data, queries and other interactions. This is the case, for example, of hospitals wanting to collaborate together to create powerful rankers to identify the cohort of patients for specific rare conditions (and as such, each hospital only holds limited data that would not be sufficient to train an effective ranker individually), but that by legislation they are forbidden to share the actual data.

To handle this issue, Federated Online Learning to Rank (FOLTR) methods have been proposed. These methods consider a decentralized machine learning scenario where data owners (clients) collaboratively train the model without sharing their data under the coordination of a central server. One such method is the Federated OLTR with Evolutionary Strategies (FOLtR-ES)~\cite{kharitonov2019federated}, which extends the OLTR optimization scenario to the Federated SGD~\cite{mcmahan2017communication} and utilizes Evolution Strategies as optimization method~\cite{salimans2017evolution}. While FOLtR-ES performs well on small-scale datasets under certain evaluation metrics, its effectiveness does not generalise to large-scale datasets and standard OLTR metrics~\cite{wang2021federated}. Because of this, we do not consider FOLtR-ES in our study. An alternative method is the FPDGD~\cite{wang2021effective}, which builds upon the state-of-the-art OLTR method, the Pairwise Differentiable Gradient Descent (PDGD)~\cite{oosterhuis2018differentiable}, and integrates it into the Federated Averaging (FedAvg) framework~\cite{mcmahan2017communication}. FPDGD exhibits effectiveness comparable to centralized OLTR methods, representing the current state-of-the-art FOLTR method. Thus, our empirical investigation of attack and defense methods on FOLTR systems relies on the FPDGD method, which is further described in Section~\ref{foltr}.
%FPDGD is empirically shown to work well than FOLtR-ES in terms of ranking effectiveness and can achieve competitive performance compared to the OLTR model trained in a centralized paradigm. 
%Later, a follow-up work by Wang et al.~\cite{wang2022non} studies the impact on FPDGD under heterogeneous local training data distribution through synthetizing typical types of non-IID data in FOLTR
%and comparing its model performance to those achieved when data is IID. Then, they investigate several existing methods on handling this issue.

 %Kharitonov et al.~\cite{kharitonov2019federated} first propose the Federated OLTR with Evolutionary Strategies (FOLtR-ES) method which extends the OLTR optimization scenario to the Federated SGD~\cite{mcmahan2017communication} and uses Evolution Strategies as the optimization method~\cite{salimans2017evolution}. Although FOLtR-ES is shown to perform well on small-scale datasets under certain evaluation metrics, the effectiveness of FOLtR-ES is not consistent across other, larger-scale datasets nor when typical OLTR metrics are considered (nDCG)~\cite{wang2021federated}. 

%To further improve the ranking performance for FOLTR system, Wang et al.~\cite{wang2021effective} propose FPDGD which leverages the state-of-the-art OLTR method, namely Pairwise Differentiable Gradient Descent (PDGD)~\cite{oosterhuis2018differentiable}, and adapts it to the Federated Averaging (FedAvg) framework~\cite{mcmahan2017communication}. FPDGD is empirically shown to work well than FOLtR-ES in terms of ranking effectiveness and can achieve competitive performance compared to the OLTR model trained in a centralized paradigm. Later, a follow-up work by Wang et al.~\cite{wang2022non} studies the impact on FPDGD under heterogeneous local training data distribution through synthetizing typical types of non-IID data in FOLTR
%and comparing its model performance to those achieved when data is IID. Then, they investigate several existing methods on handling this issue.

%To further protect the local updates from malicious attacking, FOLtR-ES also includes a privatization procedure, which leverages the theory of $\epsilon$-local differential privacy~\cite{dwork2014algorithmic}. FOLtR-ES is shown to perform well on small-scale datasets (MQ2007) for the MaxRR metric, although performance degrades when privacy preservation is required~\cite{kharitonov2019federated}. However, the effectiveness of FOLtR-ES is not consistent across other, larger-scale datasets nor when typical OLTR metrics are considered (nDCG)~\cite{wang2021federated}. 


%We have an overview of the use of federated learning in OLTR in Section~\ref{foltr}. This section also briefly introduces the FOLTR method used in our empirical experimentation for studies on poisoning attacks and defenses in this paper: the Federated Pairwise Differentiable Gradient Descent (FPDGD) method~\cite{wang2021effective}, which is
%the current state-of-the-art in FOLTR.


%\subsubsection{Other use of federated learning in Information Retrieval}
%Aside from its usage in online learning to rank,  recent works have applied federated learning in other information retrieval contexts. Zong et al.~\cite{zong2021fedcmr} provide a solution for cross-modal retrieval in a distributed data storage scenario, which uses federated learning to reduce the potential privacy risks and the high maintenance costs encountered when dealing with large amount of training data. Wang et al.~\cite{wang2021efficient} study learning to rank (but not in the online setting we consider in this article) in a cross-silo federated learning setting; this work is aimed at helping companies that have access to limited labelled data to collaboratively build a document retrieval system, in an efficient way.
%Hartmann et al.~\cite{hartmann2019federated} use federated learning to improve the ranking of suggestions
%in the Firefox URL bar, so that the training of the ranker on user interactions is performed in a privacy-preserving way; they show that this federated approach improves on the suggestions produced by the previously employed heuristics in Firefox.
%Yang et al. ~\cite{yang2018applied} describe the use of federated learning for search query suggestions in the Google Virtual Keyboard (GBoard) product. Here, a baseline model is used to identify relevant query suggestions given a user query; candidate suggestions are then filtered using a triggering model learnt using federated learning. 
%Aside from the previous examples, federated learning has also seen adoption in the area of personalised search~\cite{ghorab2013personalised}, which aims  to return search results that cater to the specific user's interests. While feature-based~\cite{carman2010towards, bennett2012modeling, harvey2013building} and deep learning-based~\cite{song2014adapting, ge2018personalizing, yao2020rlper} methods are widely used in this area, user data privacy has been often overlooked -- this is particularly the case when considering the users query logs which are collected by the central server to create the personalised ranker.  To tackle this issue, Yao et al.~\cite{yao2021fedps} recently proposed a privacy protection enhanced personalized search framework which adapts federated learning to the state-of-the-art personalized search model.

\vspace{-12pt}
\subsection{Poisoning Attacks on Federated Learning}

Poisoning attacks on federated learning systems aim to compromise the integrity of the system's global model. Poisoning attacks can be grouped according to the goals of the attack into two categories: untargeted poisoning attacks, and targeted poisoning attacks (also known as backdoor attacks).

Targeted poisoning attacks aim to manipulate a global model according to the attacker's objectives, such as misclassifying a group of data with certain features to a label chosen by the attacker, while maintaining normal model effectiveness under other conditions. This is accomplished through backdoor attacks~\cite{bagdasaryan2020backdoor, bhagoji2019analyzing}, which are designed to allow the targeted manipulations to transpire stealthily and without detection. %, while still providing high effectiveness for users.


%Targeted poisoning attacks intend to force the global model to perform in an intended way which the adversary wish the model to perform under certain adversarial condition (for example, misclassify a certain group of data with specific features to an attacker-assigned label) while at the same time, maintain the overall performance of other conditions. To achieve so, backdoor attacks~\cite{bagdasaryan2020backdoor, bhagoji2019analyzing} are designed to promote the targeted attacking stealthily while providing high-quality performance to benign users.


In contrast, untargeted poisoning attacks (also known as Byzantine failures~\cite{lamport1982byzantine, blanchard2017machine, yin2018byzantine, fang2020local, shejwalkar2021manipulating}) aim to decrease the overall effectiveness of the global model indiscriminately for all users and data groups. Current untargeted poisoning methods can be divided into two categories: data poisoning and model poisoning. 
Label flipping~\cite{biggio2012poisoning} is a representative data poisoning method:  the labels of honest training data are changed without altering their features.
Model poisoning, on the other hand, directly affects the local model updates before they are sent to the centralized server. For example, Baruch et al.~\cite{baruch2019little} poisons the local model updates through the addition of noise computed from the variance between the before-attack model updates, while Fang et al.~\cite{fang2020local}'s attacks are optimized to undermine specific robust aggregation rules. 


%Instead, for attackers who conduct untargeted poisoning (also known as Byzantine failures in some literatures~\cite{lamport1982byzantine, blanchard2017machine, yin2018byzantine, fang2020local, shejwalkar2021manipulating}), their aim is to degrade the overall performance (or effectiveness) of global model on the held-out test set. Current untargeted poisoning methods can be grouped as two types: data poisoning, model poisoning. 
%One typical data poisoning strategy is label flipping~\cite{biggio2012poisoning, tolpegin2020data}, in which the labels of honest training data of one class are flipped to another while the corresponding features maintain unchanged. Unlike data poisoning, model poisoning attacks directly compromise the local model updates before sending them to the centralised server. Baruch et al.~\cite{baruch2019little} directly poisons the local updates through adding noise computed from variance between before-attack model updates. Fang et al.~\cite{fang2020local} propose model poisoning strategies tailored to specific robust aggregation rules through formulating attacks as optimization problems. 

Among untargeted poisoning attacks on federated learning systems, model poisoning methods have been found to be the most successful~\cite{bagdasaryan2020backdoor}. In particular, data poisoning attacks have limited success when Byzantine-robust defense aggregation rules are in use~\cite{fang2020local}; we introduce these defense methods in Section~\ref{defense}.
Furthermore, most data poisoning attacks assume that the attacker has prior knowledge about the entire training dataset, which is often unrealistic in practice.

In this paper, we focus on untargeted poisoning attacks, delving into the effectiveness of both data poisoning and model poisoning methods. These attack methods are studied within the framework of a FOLTR system based on FPDGD, with and without the integration of defense countermeasures. 
%Along with attack methods, we also study the effectiveness ofunder both defensive and non-defensive settings tailored to federated online learning to rank system. 

%Previous studies have shown the evidence that model poisoning is more effective than data poisoning in FL~\cite{bagdasaryan2020backdoor}. Also, most data poisoning attacks assume that the adversary has prior knowledge about the entire training dataset, which is unfeasible in FL. Existing work has also shown that data poisoning attacks have limited success to attack Federated Learning under Byzantine-robust defensive aggregation rules~\cite{fang2020local} which we introduce in Section~\ref{defense}.





==> Chapter5_paper3_poisoning_ictir2023/sections/summary.tex <==
\section{Summary of Key Findings}

%From the empirical results presented above, we raise the following key findings:
Based on the presented empirical results above, we identify the following key findings:

\begin{itemize}
	\item In general, the perfect click type is more difficult to attack compared to the other two click models, whether it be data or model poisoning methods, except in specific instances when employing Fang's attack under the full knowledge assumption. To successfully attack a FOLTR system when perfect click feedback is present, a larger number of attackers is required due to the relatively low variance between local updates. As a result, more clients must be compromised to inject noise, otherwise the attack is more likely to be detected by robust aggregation rules.
	

\item Among all attacking strategies studied in this paper, Fang's attack with full knowledge emerged as the most successful in diminishing the performance of the global model, though some exceptions were observed in the noisy informational click scenario. When there were more malicious clients (i.e. 30\% or 40\% of the total clients), Fang's attack with partial knowledge is just as effective as with full knowledge. This indicates that model poisoning is more effective than data poisoning. Furthermore, when defense measures were implemented, Fang's attack demonstrated greater success against Krum and Multi-Krum aggregation rules in comparison to Trimmed Mean and Median.

	
%	\item Among all attacking strategies studied in this paper, Fang's attack under full knowledge performs consistently better in compromising the effectiveness of global model except for some scenarios under the noisiest \textit{informational} click. With more attackers involving (i.e. 30\%, 40\%), Fang's attack with partial knowledge can achieve similar attacking utility as under full knowledge scenario. This demonstrates the superiority of model poisoning than data poisoning. Under defensive situation, Fang's attack works well on Krum and Multi-Krum aggregation rules than Trimmed Mean and Median.
	
%	\item Although Krum have shown its effectiveness in defending against data poisoning while Timmed Mean on detecting Fang's attack, more attention should be paid when deploying Krum and Trimmed Mean as the utility drops under no-attacker system brought by those two aggregation rules.
	
\item It is essential to highlight that although Krum has proven effective in countering data poisoning and Trimmed Mean in defending against Fang's attack, deploying these two aggregation rules should be exercised with caution as they result in an overall decrease in search performance if the system is not exposed to attacks. Thus, the selection of these defense mechanisms should be carefully considered, taking into account the specific context and risk of potential attacks to strike the right balance between security and search effectiveness.


%It is essential to highlight that while Krum has proven effective in countering data poisoning and Trimmed Mean in defending against Fang's attack, deploying these two aggregation rules should be exercised with caution. It has been observed that they lead to an overall decrease in search performance when the system is not subjected to attacks. Thus, the selection of these defense mechanisms should be carefully considered, taking into account the specific context and risk of potential attacks to strike the right balance between security and search effectiveness.
\end{itemize}

==> Chapter6_paper4_unlearning_ecir2024/sections/related-works.tex <==
\section{Related Work}

%\subsubsection*{Federated Online Learning to Rank.}
\textbf{Federated Online Learning to Rank.}
% \textbf{Federated Online Learning to Rank.}
FOLTR systems consider a decentralized OLTR~\cite{hofmann2013reusing,schuth2016multileave,zhao2016constructing,oosterhuis2018differentiable,wang2018efficient,zhuang2020counterfactual,zhuang2022reinforcement,jia2022learning} scenario where data owners (clients) collaboratively train a ranker in an online manner under the coordination of a central server without the need of sharing their data. 
Though FOLTR is still largely unexplored, few existing works have established an initial landscape of this research area.
%
The Federated OLTR with Evolutionary Strategies (FOLtR-ES)~\cite{kharitonov2019federated} method was the first FOLTR system proposed in the literature. FOLtR-ES extends the centralised OLTR scenario into federated setting~\cite{mcmahan2017communication} and uses Evolution Strategies as optimization method~\cite{salimans2017evolution}. 
%
While FOLtR-ES performs well on small-scale datasets under specific evaluation metrics, its effectiveness does not generalize to large-scale datasets and standard OLTR metrics~\cite{wang2021federated}.
%
To improve the effectiveness of FOLTR, Wang et al.~\cite{wang2021effective} proposed an alternative method named FPDGD~\cite{wang2021effective}, which leverages the state-of-the-art OLTR method, the Pairwise Differentiable Gradient Descent (PDGD)~\cite{oosterhuis2018differentiable}, and adapts it to the Federated Averaging (FedAvg) framework~\cite{mcmahan2017communication}. 
FPDGD's effectiveness is comparable to that of centralized OLTR methods and is currently the state-of-the-art FOLTR method.
%
Though, we noticed that Wang et al.~\cite{wang2022non} pointed out that FPDGD's effectiveness has been shown to deteriorate if data is not distributed identically and independently (non-IID) across clients. 


%% security of parameters
%Although the parameters of a federated learning model do not directly reveal users' private data, they can be attacked to reveal sensitive information about that data~\cite{DBLP:conf/ccs/FredriksonJR15,DBLP:conf/nips/GeipingBD020}.
%%
%To add a stronger privacy guarantee to FOLTR systems, Wang et al.~\cite{wang2021effective} proposed a method to secure the model parameters of FPDGD based on differential privacy. The use of differential privacy, however, degrades the effectiveness of the ranker. \todo{I suggest to remove this paragraph as it is not related to this paper}


This paper extends the landscape of existing works by adding an unlearning mechanism to a FOLTR system.
In our experiments we use FPDGD~\cite{wang2021effective} as the base FOLTR system. 
To avoid entangling different sources of challenges, we do not consider non-IID settings~\cite{wang2022non} and  privacy-preserving mechanisms~\cite{wang2021effective} within unlearning in our experiments.
The study of unlearning across these more complex experimental settings is left for future work.



% non-iid
%In addition, Wang et al.~\cite{wang2022non} have highlighted that the ranker may be negatively affected by data that is not identically and independently distributed across different clients.

%Furthermore, Wang et al.~\cite{wang2022non} pointed out that non-IID data across different clients can hurt the performance of ranker.
%%
%The existing works have not considered a FOLTR-exit mechanism yet, and we thus explore unlearning for FOLTR to complement current research.


%\vspace{-10pt}
%\subsubsection*{Machine Unlearning.}
% \noindent
% \textbf{Machine Unlearning.}

\textbf{Machine Unlearning.} Our work is related to machine unlearning~\cite{bourtoule2021machine,nguyen2022survey}, which pertains to the removal of any evidence of a chosen data point from the model, a process commonly known as selective amnesia. Except ensuring the removal of certain data points from the model being the primary objective, the unlearning procedure should also do not affect the model's effectiveness. Machine unlearning has been explored in both centralised~\cite{DBLP:conf/sp/CaoY15,bourtoule2021machine} and federated settings~\cite{liu2021federaser,halimi2022federated,wang2022federated,che2023fast}, but never for FOLTR -- this is a novel contribution of our work. 
%

Methods in machine unlearning can be broadly classified into two families: exact unlearning and approximate unlearning. Exact unlearning methods are designed to provide a theoretical guarantee that the methods can completely remove the influence of the data to be forgotten~\cite{DBLP:journals/ml/BaumhauerSZ22,DBLP:conf/icml/BrophyL21,DBLP:journals/cluster/ChenXXZ19,DBLP:conf/nips/GinartGVZ19,mahadevan2021certifiable}; but a limitation of these methods is that they can only be applied to simple machine learning models.
%Some works~\cite{DBLP:journals/ml/BaumhauerSZ22,DBLP:conf/icml/BrophyL21,DBLP:journals/cluster/ChenXXZ19,DBLP:conf/nips/GinartGVZ19} studied exact unlearning methods which are designed to theoretically guarantee that models can totally remove the influence of removed data but can only be applied to simple methods.
Approximate unlearning methods, on the other hand,  are characterized by higher efficiency, which is achieved by relying on specific assumptions regarding the accessibility of training information, and by permitting a certain amount of reduction in the model's effectiveness~\cite{DBLP:journals/access/AldaghriMB21,DBLP:conf/ccs/Chen000H022,chundawat2023zero}.
These methods can be used on more complex machine learning models (e.g., deep neural networks). 
%On the contrary, some other works~\cite{DBLP:journals/access/AldaghriMB21,DBLP:conf/ccs/Chen000H022} investigated approximate unlearning, which can achieve unlearning in more complex models like neural networks.
%
The existing unlearning methods for federated learning belong to the approximate unlearning family~\cite{liu2021federaser,DBLP:journals/corr/abs-2003-10933,DBLP:conf/infocom/LiuXYWL22}: our method builds upon one such methods, FedEraser~\cite{liu2021federaser}.
However, most of these methods are applied to classification tasks and no previous work considers either ranking or FOLTR systems.
%Our method is migrated from FedEraser~\cite{liu2021federaser}.

%\todo{split the section or not?}
%\subsubsection*{Evaluation of Machine Unlearning.}
\textbf{Evaluation of Machine Unlearning.}
A key challenge posed by the task of unlearning in the federated learning context is how to evaluate whether an unlearning method has successfully removed the contributions from the client that requested to leave the federation. This evaluation is at times termed as unlearning verification~\cite{nguyen2022survey}, which specifically aims to certify that the unlearned model is unrelated to the data that needed to be removed. 
Due to the stochastic nature of the training for many machine learning models, it is difficult to distinguish the individual clients' models and their unlearned counterparts after a certain group of data is removed. 

To evaluate the effectiveness of unlearning, a group of methods leverage membership inference attacks~\cite{liu2021federaser,chen2021machine,hu2022membership}, i.e. a kind of attack method that predicts whether a data item belongs to the training data of a certain model~\cite{shokri2017membership}: it is then straightforward to adapt this type of attacks to verify if the unlearned samples participated in the unlearning process. However, conducting successful membership inference attacks needs subtle design and training of the inference model. The effectiveness of such attacks on FOLTR is unknown as it is an unexplored area. Thus, we do not consider this type of verification in our study.

Another type of methods is inspired from the idea of poisoning attacks; in our experiments, we embrace this direction for evaluating unlearning. 
These methods add arbitrary noise~\cite{yuan2023federated} or backdoor triggers~\cite{gao2022verifi,sommer2022athena,wu2022federated,halimi2022federated} to the data that is needed to be deleted, with the aim of manipulating the effectiveness of the trained model. After the unlearning of poisoned datasets has taken place, the impact from the arbitrary poisoning or backdoor triggers should be reduced in the unlearned model: the extent of this reduction (and thus model gains) determines the extent of the success of unlearning.

A significant difference between our work and existing unlearning works is that we consider the context of FOLTR, which has specific challenges not present in common classification tasks (e.g., ranking vs. classification, online learning vs. offline learning, etc.). Thus, methods proposed in the general machine learning community may not work in FOLTR. 
Instead of diving into a specific problem, we establish the first unlearning benchmark -- including both unlearning method and evaluation setting -- for FOLTR. By doing so, we 
%help diversify the evaluation settings of general federated unlearning methods, and 
facilitate future works which focus on the specific challenges of unlearning in FOLTR.



%
%\todo{Besides methods that studies conducting unlearning effectively, evaluation on the success of unlearning is also important. Due to the stochastic factors in the training of machine learning models, it is difficult to distinguish the model and its unlearned counterparts after a certain group of data is removed. The evaluation process is also termed as unlearning verification~\cite{nguyen2022survey}, with the aim of certifying that the unlearn models is unrelated to the data to be removed. To evaluate the effectiveness of unlearning, a group of methods leverage membership inference attacks~\cite{liu2021federaser, chen2021machine, hu2022membership}, i.e. a kind of attack methods that predict whether a data item belongs to the training data of a certain model~\cite{shokri2017membership}. Thus, it is straightforward to adapt this type of attacks to verify if the unlearned samples participate in the unlearning process. Another type of methods is inspired from the idea of poisoning attacks. With the aim of manipulating the performance of the trained model, arbitrary noise~\cite{yuan2023federated} or backdoor triggers~\cite{gao2022verifi, sommer2022athena, wu2022federated, halimi2022federated} are added to the data that is to be deleted. After unlearning the poisoned datasets, the impact from arbitrary poisoning or backdoor triggers should be reduced in the unlearned model.} 

==> Chapter6_paper4_unlearning_ecir2024/sections/sections/related-works.tex <==
\section{Related Work}

\subsection{Federated Online Learning to Rank}
% \textbf{Federated Online Learning to Rank.}
FOLTR systems consider a decentralized OLTR~\cite{hofmann2013balancing,hofmann2013reusing,schuth2016multileave,zhao2016constructing,oosterhuis2018differentiable,wang2018efficient,zhuang2020counterfactual,zhuang2021online,jia2021pairrank,oosterhuis2021unifying,zhuang2022reinforcement,jia2022learning} scenario where data owners (clients) collaboratively train a  ranker in an online manner under the coordination of a central server without the need of sharing their data. 
% effectiveness
% While online training of rankers has been largely explored~\cite{hofmann2013balancing,hofmann2013reusing,schuth2016multileave,zhao2016constructing,oosterhuis2018differentiable,wang2018efficient,zhuang2020counterfactual,zhuang2021online,jia2021pairrank,oosterhuis2021unifying,zhuang2022reinforcement,jia2022learning}, the training of these rankers within a federated system is still largely unexplored. 
Though FOLTR is still largely unexplored, few existing works have established an initial landscape of this research area.
%
The Federated OLTR with Evolutionary Strategies (FOLtR-ES)~\cite{kharitonov2019federated} method was the first FOLTR system proposed in the literature. FOLtR-ES extends the centralised OLTR scenario into federated setting~\cite{mcmahan2017communication} and uses Evolution Strategies as optimization method~\cite{salimans2017evolution}. 
%
While FOLtR-ES performs well on small-scale datasets under specific evaluation metrics, its effectiveness does not generalize to large-scale datasets and standard OLTR metrics~\cite{wang2021federated}.
%
To improve the effectiveness of FOLTR, Wang et al.~\cite{wang2021effective} proposed an alternative FOLTR method FPDGD~\cite{wang2021effective}, which leverages the state-of-the-art OLTR method, the Pairwise Differentiable Gradient Descent (PDGD)~\cite{oosterhuis2018differentiable}, and adapts it to the Federated Averaging (FedAvg) framework~\cite{mcmahan2017communication}. 
FPDGD's effectiveness is comparable to that of centralized OLTR methods and is currently the state-of-the-art FOLTR method.
%
Though, we noticed that Wang et al.~\cite{wang2022non} pointed out that FPDGD's effectiveness has been shown to deteriorate if data is not distributed identically and independently (non-IID) across clients. 


%% security of parameters
%Although the parameters of a federated learning model do not directly reveal users' private data, they can be attacked to reveal sensitive information about that data~\cite{DBLP:conf/ccs/FredriksonJR15,DBLP:conf/nips/GeipingBD020}.
%%
%To add a stronger privacy guarantee to FOLTR systems, Wang et al.~\cite{wang2021effective} proposed a method to secure the model parameters of FPDGD based on differential privacy. The use of differential privacy, however, degrades the effectiveness of the ranker. \todo{I suggest to remove this paragraph as it is not related to this paper}


This paper extends the landscape of existing works by adding an unlearning mechanism to a FOLTR system.
In our experiments we use FPDGD~\cite{wang2021effective} as the base FOLTR system. 
To avoid entangling different sources of challenges, we do not consider non-IID settings~\cite{wang2022non} and  privacy-preserving mechanisms~\cite{wang2021effective} within unlearning in our experiments.
The study of unlearning across these more complex experimental settings is left for future work.



% non-iid
%In addition, Wang et al.~\cite{wang2022non} have highlighted that the ranker may be negatively affected by data that is not identically and independently distributed across different clients.

%Furthermore, Wang et al.~\cite{wang2022non} pointed out that non-IID data across different clients can hurt the performance of ranker.
%%
%The existing works have not considered a FOLTR-exit mechanism yet, and we thus explore unlearning for FOLTR to complement current research.


%\vspace{-10pt}
\subsection{Machine Unlearning}
% \noindent
% \textbf{Machine Unlearning.}
Our work is related to the area of machine unlearning~\cite{nguyen2022survey}, which pertains to the removal of any evidence of a chosen data point from the model, a process commonly known as selective amnesia. The primary objective of this procedure is to ensure that the model's effectiveness is not affected. Machine unlearning has been explored in both centralised~\cite{DBLP:conf/sp/CaoY15} and federated settings~\cite{liu2021federaser}, but never in the context of FOLTR -- this is a novel contribution of this paper. 
%

Methods in machine unlearning can be broadly classified into two families: exact unlearning and approximate unlearning. Exact unlearning methods are designed to provide a theoretical guarantee that the methods can completely remove the influence of the data to be forgotten~\cite{DBLP:journals/ml/BaumhauerSZ22,DBLP:conf/icml/BrophyL21,DBLP:journals/cluster/ChenXXZ19,DBLP:conf/nips/GinartGVZ19,mahadevan2021certifiable}; but a limitation of these methods is that they can only be applied to simple machine learning models.
%Some works~\cite{DBLP:journals/ml/BaumhauerSZ22,DBLP:conf/icml/BrophyL21,DBLP:journals/cluster/ChenXXZ19,DBLP:conf/nips/GinartGVZ19} studied exact unlearning methods which are designed to theoretically guarantee that models can totally remove the influence of removed data but can only be applied to simple methods.

Approximate unlearning methods, on the other hand,  are characterized by higher efficiency, which is achieved by relying on specific assumptions regarding the accessibility of training information, and by permitting a certain amount of reduction in the model's effectiveness~\cite{DBLP:journals/access/AldaghriMB21,DBLP:conf/ccs/Chen000H022,chundawat2022zero}.
These methods can be used on more complex machine learning models (e.g., deep neural networks). 
%On the contrary, some other works~\cite{DBLP:journals/access/AldaghriMB21,DBLP:conf/ccs/Chen000H022} investigated approximate unlearning, which can achieve unlearning in more complex models like neural networks.
%
The existing unlearning methods for federated learning belong to the approximate unlearning family~\cite{liu2021federaser,DBLP:journals/corr/abs-2003-10933,DBLP:conf/infocom/LiuXYWL22}: our method builds upon one such methods, FedEraser~\cite{liu2021federaser}.
However, most of these methods are applied to classification tasks and no previous work considers either ranking or FOLTR systems.
%Our method is migrated from FedEraser~\cite{liu2021federaser}.

%\todo{split the section or not?}
\subsection{Evaluation of Machine Unlearning}
A key challenge posed by the task of unlearning in the federated learning context is how to evaluate whether an unlearning method has successfully removed the contributions from the client that requested to leave the federation. This evaluation is at times termed as unlearning verification~\cite{nguyen2022survey}, which specifically aims to certify that the unlearned model is unrelated to the data that needed to be removed. 
Due to the stochastic nature of the training of many machine learning models, including deep learning approaches, it is difficult to distinguish the individual clients' models and their unlearned counterparts after a certain group of data is removed. 

To evaluate the effectiveness of unlearning, a group of methods leverage membership inference attacks~\cite{liu2021federaser, chen2021machine, hu2022membership}, i.e. a kind of attack method that predicts whether a data item belongs to the training data of a certain model~\cite{shokri2017membership}: it is then straightforward to adapt this type of attacks to verify if the unlearned samples participated in the unlearning process. However, conducting successful membership inference attacks needs subtle design and training of the inference model. The effectiveness of such attacks on FOLTR is unknown as it is an unexplored area. Thus, we do not consider this type of verification in our study.

Another type of methods is inspired from the idea of poisoning attacks; in our experiments, we embrace this direction for evaluating unlearning. 
These methods add arbitrary noise~\cite{yuan2023federated} or backdoor triggers~\cite{gao2022verifi, sommer2022athena, wu2022federated, halimi2022federated} to the data that is needed to be deleted, with the aim of manipulating the effectiveness of the trained model. After the unlearning of the now poisoned datasets has taken place, the impact from the arbitrary poisoning or backdoor triggers should be reduced in the unlearned model: the extent of this reduction (and thus model gains) determines the extent of the success of the unlearning process.

A significant difference between our work and these existing unlearning works is that we are located in the context of FOLTR, which has specific challenges that are not present in common classification tasks (e.g., ranking vs. classification, online learning vs. offline learning, etc.). This means the methods proposed in the general machine learning community may not work in FOLTR. 
Instead of diving into a specific problem, we establish the first unlearning benchmark -- including both unlearning method and evaluation setting -- for FOLTR. By doing so, we help diversify the evaluation settings of general federated unlearning methods, and facilitate future works which focus on the specific challenges of unlearning in FOLTR.



%
%\todo{Besides methods that studies conducting unlearning effectively, evaluation on the success of unlearning is also important. Due to the stochastic factors in the training of machine learning models, it is difficult to distinguish the model and its unlearned counterparts after a certain group of data is removed. The evaluation process is also termed as unlearning verification~\cite{nguyen2022survey}, with the aim of certifying that the unlearn models is unrelated to the data to be removed. To evaluate the effectiveness of unlearning, a group of methods leverage membership inference attacks~\cite{liu2021federaser, chen2021machine, hu2022membership}, i.e. a kind of attack methods that predict whether a data item belongs to the training data of a certain model~\cite{shokri2017membership}. Thus, it is straightforward to adapt this type of attacks to verify if the unlearned samples participate in the unlearning process. Another type of methods is inspired from the idea of poisoning attacks. With the aim of manipulating the performance of the trained model, arbitrary noise~\cite{yuan2023federated} or backdoor triggers~\cite{gao2022verifi, sommer2022athena, wu2022federated, halimi2022federated} are added to the data that is to be deleted. After unlearning the poisoned datasets, the impact from arbitrary poisoning or backdoor triggers should be reduced in the unlearned model.} 

==> PreliminaryAndBackPages/Back.tex <==
% ***************************************************
% Back Matter
% ***************************************************
% ADD AN ENDQUOTE HERE. If you do not wish to, delete this file.
\backmatter

\normalfont
\cleartooddpage

\pagestyle{empty}

\begin{table}[b!]
\begin{center}
% ********* Enter your quote within {} brackets: ********
\textit{Endquote goes here.}

% ********************************************************
\end{center}
\begin{flushright}
% ********* Enter your text below, as indicated: ********
Author of quote,\\
Source of quote

% ********************************************************
\end{flushright}
\end{table}
